INSPIRIT: Optimizing Heterogeneous Task Scheduling through Adaptive Priority in Task-based Runtime Systems

As modern HPC computing platforms become increasingly heterogeneous, it is challenging for programmers to fully leverage the computation power of massive parallelism offered by such heterogeneity. Consequently, task-based runtime systems have been proposed as an intermediate layer to hide the complex heterogeneity from the application programmers. The core functionality of these systems is to realize efficient task-to-resource mapping in the form of Directed Acyclic Graph (DAG) scheduling. However, existing scheduling schemes face several drawbacks to determine task priorities due to the heavy reliance on domain knowledge or failure to efficiently exploit the interaction of application and hardware characteristics. In this paper, we propose INSPIRIT, an efficient and lightweight scheduling framework with adaptive priority designed for task-based runtime systems. INSPIRIT introduces two novel task attributes \textit{inspiring ability} and \textit{inspiring efficiency} for dictating scheduling, eliminating the need for application domain knowledge. In addition, INSPIRIT jointly considers runtime information such as ready tasks in worker queues to guide task scheduling. This approach exposes more performance opportunities in heterogeneous hardware at runtime while effectively reducing the overhead for adjusting task priorities. Our evaluation results demonstrate that INSPIRIT achieves superior performance compared to cutting edge scheduling schemes on both synthesized and real-world task DAGs.

==> artifact.tex <==
%\onecolumn
\section*{Paper Artifact Description Appendix}
\label{sec:AD}

{\color{orange}\textit{Computational Artifacts:}} Yes

\subsection*{Artifact Description Details}

\noindent {\color{orange}\textbf{\textit{Summarize the experiments reported in the paper and how they were run.}}}

The evaluation scripts and source codes can be downloaded from the link given in \textit{Artifact 1}. The compared state-of-the-art implementations, including Ansor, AutoTVM, and XLA, are all in this repository. The evaluation source codes and scripts of motivation experiments are also included in this repository.
In summary, one can build FamilySeer and other compared implementations with the build script \texttt{build.sh} and run all evaluations following \texttt{README.md} and \texttt{scripts/README.md}.
The evaluation results will be generated in \texttt{scripts/evaluation\_result}.

\noindent {\color{orange}\textit{Software Artifact Availability:}} The source code of FamilySeer can be downloaded from the following link.

\url{https://github.com/noobotdj/tvm}


\noindent {\color{orange}\textit{Hardware Artifact Availability:}} Not publicly available.

\noindent {\color{orange}\textit{Data Artifact Availability:}} The input data used in the evaluation can be checked from the following link.

\url{https://github.com/noobotdj/tvm/FamilySeer-artifact}

\noindent {\color{orange}\textit{Proprietary Artifacts:}} None.

\noindent {\color{orange}\textit{Author-Created or Modified Artifacts:}}

\textit{Artifact 1}

Persistent ID: \url{https://github.com/noobotdj/tvm/FamilySeer-artifact}

Artifact name: Evaluation scripts and source codes of FamilySeer.

\noindent {\color{orange}\textit{Operating systems and versions:}} The CPU and GPU platforms are installed with 64-bit Ubuntu v20.04.

\noindent {\color{orange}\textit{Compilers and versions:}} GCC 9.3 and LLVM v8.0.0.

\noindent {\color{orange}\textit{Libraries and versions:}} CUDA 11.2.

\noindent {\color{orange}\textit{Input datasets and versions:}} Random input tensors with specific shapes corresponding to different DL models. Refer to \textit{artifact 1}.


==> overview.tex <==
\section{Design Overview}
\label{sec:overview}
To address the above drawbacks, we propose a new auto-tuning framework, FamilySeer, that exploits subgraph similarity to better train the cost models and allocate time budgets for improved search quality and efficiency. The design overview of FamilySeer is shown in Figure~\ref{fig:overview}, which contains two parts such as identifying subgraph families and foresee tuning. FamilySeer takes the DL model as the input and obtains a series of subgraphs according to the graph partition rules (\eg, rules provided by TVM). Then, it clusters the subgraphs into several families according to the subgraph similarities, where the subgraphs in a family can share the training samples. FamilySeer then tunes the subgraph families by generating program candidates and selecting the candidates with better performance in an iterative manner.

\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{figure/overview.pdf}
	\caption{Design overview of FamilySeer, including two main parts: identifying subgraph families and foresee tuning.}
	\label{fig:overview}
\end{figure*}

The subgraph family is the foundation for the improvement of FamilySeer's search quality and efficiency. With the subgraphs clustered into different subgraph families, individual cost models are trained at subgraph family basis and can achieve higher model accuracy. Then, the cost models are used to accurately estimate the latency of generated program candidates for subgraphs within a family. To achieve low overhead of subgraph clustering, we measure the subgraph similarity based on easy-to-obtain attributes such as the core operator, the number of operators, and the operator sequence. 
Similar to traditional search techniques such as Ansor, (\ding{172}) FamilySeer starts with the most bottleneck subgraph and picks up its program candidates with high performance potential, which is estimated by the cost model of the family it belongs to. 
Generally, the subgraphs with higher latency have higher improving potential, and the subgraph with the highest potential can be regarded as the bottleneck subgraph.
These program candidates are sent to real hardware (\eg, GPUs) for latency measurement, and the results are returned to the subgraph family, which are then used to train the cost model to improve its accuracy. 

% 在这里解释Family cost model
After identifying subgraph families, the cost models are built at subgraph family basis, and they are necessary for estimating the performance of generated program candidates. Accurate cost models can help to identify program candidates with high performance potential, eliminating the latency measurements of program candidates on real hardware. 
For the design of family cost model, we adopt the gradient boosting decision tree  (\eg, XGBoost). Specifically, the family cost model extracts the computation and memory access features (similar to Ansor~\cite{zheng2020ansor}) from program candidates, and builds feature vectors to estimate the latency of the program candidates. By feeding in different training samples (\ie, program candidates belonging to the corresponding family), the cost models can be trained at subgraph family basis.

The foresee tuning further optimizes the search process targeting subgraph families. Different from traditional search techniques, (\ding{173}) it then picks another bottleneck subgraph within the same family as previous subgraph for program search. The cost model per subgraph family is used again to estimate the high potential program candidates for hardware measurements. Since subgraphs within a family are similar, the cost model can accurately identify high quality program candidates without selecting numerous candidates for costly hardware measurements. The measurements are also sent back to subgraph family and used to train its cost model. The above procedure (\ding{172} + \ding{173}) is executed iteratively until the time budget is expired. Due to the advantage of reducing the number of costly hardware measurements significantly while maintaining high search quality for program candidates, FamilySeer not only improves search efficiency within a limited time budget, but also improves search quality with more accurate cost models across subgraph families. 
